Springer Motives

We show that the motive of a Springer fiber is pure Tate. We then consider a category of equivariant Springer motives on the nilpotent cone and construct an equivalence to the derived category of graded modules over the graded affine Hecke algebra.

==> Inhalt/Result.tex <==
%!TEX root = ../main.tex
